Explaining Time Series Predictions with Dynamic Masks

How can we explain the predictions of a machine learning model? When the data is structured as a multivariate time series, this question induces additional difficulties such as the necessity for the explanation to embody the time dependency and the large number of inputs. To address these challenges, we propose dynamic masks (Dynamask). This method produces instance-wise importance scores for each feature at each time step by fitting a perturbation mask to the input sequence. In order to incorporate the time dependency of the data, Dynamask studies the effects of dynamic perturbation operators. In order to tackle the large number of inputs, we propose a scheme to make the feature selection parsimonious (to select no more feature than necessary) and legible (a notion that we detail by making a parallel with information theory). With synthetic and real-world data, we demonstrate that the dynamic underpinning of Dynamask, together with its parsimony, offer a neat improvement in the identification of feature importance over time. The modularity of Dynamask makes it ideal as a plug-in to increase the transparency of a wide range of machine learning models in areas such as medicine and finance, where time series are abundant.

==> Parts/related.tex <==



\iffalse 
Finally, Dynamask provides an explanation for each prediction. This property is often referred to as \emph{instance-wise explainability} in the literature~\citep{Baehrens2010, Yang2018, Yoon2019, Tonekaboni2020}.

Dynamask uses the model as a black-box without paying attention to its nature or architecture~\footnote{We only need the black-box to be differentiable with respect to its input.}, it can thus be considered as a model agnostic method.  Another interesting characteristic of Dynamask is that it does not require the knowledge of the training set from which the black-box was obtained. This training set agnosticity (abbreviated Train agnostic in Table~\ref{table-related})) protects our method from overfitting. 

\fi

==> Parts/related_details.tex <==
In this section, we elaborate on the different type of saliency methods encountered in the literature. We distinguish them according to the way they interact with a model to produce importance scores.

\textbf{Gradient-based} These methods use the gradient of the model's prediction with respect to the features to produce importance scores. The premise is the following: if a feature is salient, we expect it to have a big impact on the model's prediction when varied locally. This translates into a big gradient of the model's output with respect to this feature. Popular gradient methods include Integrated Gradient~\citep{Sundararajan2017}, DeepLIFT~\citep{Shrikumar2017} and GradSHAP~\citep{Lundberg2018}. 

\textbf{Perturbation-based} These methods use the effect of a perturbation in the input on the model's prediction to produce importance scores. The premise is similar to the one used in gradient based method. The key difference lies in the way in which the feature is varied. If gradient based methods use local variation of the features (according to the gradient), perturbation-based method use the data itself to produce a variation. Popular examples include Feature Occlusion\citep{Suresh2017} that replace a group of features with a baseline or Feature Permutation that performs individual permutation of features within a batch.

\textbf{Interpretable by architecture} For some models, the architecture allows to perform simple explainability tasks, such as determining feature saliency. A popular example, building on the success attention mechanisms~\citep{Vaswani2017}, is the usage of attention layers to produce importance scores~\citep{Choi2016, Song2017, Xu2018, Kwon2018}. It should be noted that this approach has already been criticized~\citep{Jain2019}.

\textbf{Other} There are some methods, such as SHAP~\citep{Lundberg2017}, FIT~\citep{Tonekaboni2020}, LIME~\citep{Ribeiro2016} or INVASE~\citep{Yoon2019} that don't clearly fit in one of the above categories.

